Likelihood-Free Frequentist Inference: Bridging Classical Statistics and Machine Learning for Reliable Simulator-Based Inference

Many areas of science rely on simulators that implicitly encode intractable likelihood functions of complex systems. Classical statistical methods are poorly suited for these so-called likelihood-free inference (LFI) settings, especially outside asymptotic and low-dimensional regimes. At the same time, popular LFI methods - such as Approximate Bayesian Computation or more recent machine learning techniques - do not necessarily lead to valid scientific inference because they do not guarantee confidence sets with nominal coverage in general settings. In addition, LFI currently lacks practical diagnostic tools to check the actual coverage of computed confidence sets across the entire parameter space. In this work, we propose a modular inference framework that bridges classical statistics and modern machine learning to provide (i) a practical approach for constructing confidence sets with near finite-sample validity at any value of the unknown parameters, and (ii) interpretable diagnostics for estimating empirical coverage across the entire parameter space. We refer to this framework as likelihood-free frequentist inference (LF2I). Any method that defines a test statistic can leverage LF2I to create valid confidence sets and diagnostics without costly Monte Carlo or bootstrap samples at fixed parameter settings. We study two likelihood-based test statistics (ACORE and BFF) and demonstrate their performance on high-dimensional complex data. Code is available at https://github.com/lee-group-cmu/lf2i.

==> sections/sources_of_error.tex <==
In traditional statistical inference, confidence sets depend on the choice of  test statistic, the assumed distribution of the test statistic under the null, and the amount of available data. In LFI, however, there are additional sources of errors. For our  LF2I  inference machinery, we categorize these errors as follows:
\begin{enumerate}
    \item[$e_1$:] Estimation error in learning the odds (Section~\ref{sec:learn_odds});
    \item[$e_2$:] Numerical error in evaluating the test statistic by maximization in \ACORE (Equation~\ref{eq:ACORE_statistic}) or by integration in \BFF (Equation~\ref{eq:BFF_statistic}); 
    \item[$e_3$:] Estimation error in learning the critical values (Section~\ref{sec:critical-value}) or the p-values (Section~\ref{sec:pval}).
\end{enumerate}
\revJMLR{{\bf Validity and power.}}  {\em Validity} is directly determined by $e_3$. As shown in Section~\ref{sec:theory}, one can construct valid confidence sets regardless of how well the test statistic is estimated, as long as the quantile regressor (Algorithm~\ref{alg:estimate_cutoffs}) or probabilistic classifier for estimating p-values  (Algorithm~\ref{alg:estimate_pvalues})  is consistent and the training sample size $B'$ is large enough. The {\em power or expected size} of the confidence set is, \revJMLR{on the other hand}, determined by both $e_1$ and $e_2$.  The error $e_1$ depends on the capacity of the classifier for estimating odds and the training sample size  $B$. The error $e_2$ is a purely numerical error and can be reduced by increasing the computational budget. \revJMLR{Note that in the examples in Section~\ref{sec:examples}, we are not employing any particular optimization or importance-weighted integration technique; we are simply generating a uniform grid over the parameter space and then computing the maximum or sum of relevant quantities over the grid points to evaluate the \ACORE or \BFF statistics, respectively.}\\
\\
\revJMLR{{\bf Practical Strategy.}} To mitigate all sources of errors, we 
\revJMLR{choose learning methods, number of simulations, and number of grid points as follows}:
\begin{enumerate}
    \item
    \revJMLR{To estimate the odds function,} select a probabilistic classifier and \revJMLR{the number of simulations} $B$ 
    based on the cross-entropy loss on held-out data;\footnote{ \revJMLR{One can alternatively} use  the integrated odds loss (Equation~\ref{eq::odds_loss}). However, as shown in Supplementary Material~\ref{app:sim_derivs}, the odds loss is much more sensitive than the cross-entropy loss to the value of the estimated odds, \revJMLR{which can lead to the odds loss wildly fluctuating for different values of $B$.}}
     \item
     \revJMLR{To compute the test statistic,} choose the number of  \revJMLR{grid points for the numerical integration or optimization} based on \revJMLR{the available} computational budget;
     \item
     \revJMLR{To ensure valid confidence sets,} select the quantile regressor and the train sample size $B'$ \revJMLR{so that we} achieve nominal coverage across \revJMLR{the entire} parameter space according to \revJMLR{LF2I diagnostics (Section~\ref{sec:diagnostics}).} 
\end{enumerate}
